Exploiting Label Skews in Federated Learning with Model Concatenation

Federated Learning (FL) has emerged as a promising solution to perform deep learning on different data owners without exchanging raw data. However, non-IID data has been a key challenge in FL, which could significantly degrade the accuracy of the final model. Among different non-IID types, label skews have been challenging and common in image classification and other tasks. Instead of averaging the local models in most previous studies, we propose FedConcat, a simple and effective approach that concatenates these local models as the base of the global model to effectively aggregate the local knowledge. To reduce the size of the global model, we adopt the clustering technique to group the clients by their label distributions and collaboratively train a model inside each cluster. We theoretically analyze the advantage of concatenation over averaging by analyzing the information bottleneck of deep neural networks. Experimental results demonstrate that FedConcat achieves significantly higher accuracy than previous state-of-the-art FL methods in various heterogeneous label skew distribution settings and meanwhile has lower communication costs. Our code is publicly available at https://github.com/sjtudyq/FedConcat.

==> del/conclusion.tex <==
\section{Conclusion}
\label{sec:con}

In this paper, we propose to alleviate the accuracy decay induced by label skews in FL through concatenation. We show that in most cases, our methods can significantly outperform various state-of-the-art FL algorithms with smaller communication costs. %\YQ{Our framework can be also combined with other state-of-the-art FL methods.} %This framework is orthogonal with other improvement in FL training. For example, we can use MOON instead of FedAvg when training encoders. Client selection strategies can be applied to FedConcat too. Though our experiments focus on vision tasks, FedConcat can also be extended to RNN to solve time-series tasks. 
FedConcat can alleviate accuracy decay because it divides the hard problem (training a model among all clients under extreme label skews) into various easy problems (training one model within each cluster under alleviated label skews). Then it collects clues of easy problems (i.e., extracted features) to solve the hard original problem. Our approach brings new insights to the FL community to look for other aggregation approaches instead of averaging.
% Therefore, FedConcat can hardly improve the result of FedAvg under IID settings. 

% For future work, it is rewarding to find some adaptive way to perform clustering based on participants' data. It is also interesting to explore assigning different models for different clusters according to data quantity and computational resources. Our framework allows for such flexibility. 

==> del/discussion.tex <==
\section{Discussion}

\subsection{Clients with only one label}
FedConcat, as well as aforementioned benchmark FL algorithms, does not work for clients with only one label, i.e. $\#C=1$ partition in \cite{li2021federated}. According to experiments, if a neural network is trained on some client with only one label for a few epochs, its loss becomes zero and such network consistently predicts that label regardless of input. This can be explained by the information bottleneck theory \cite{Tishby2015DeepLA}. Since there is only one label, the network can forget everything related to the feature and directly output that label. Thus many FL algorithms cannot work well for such extreme non-IID case. 

There are some research \cite{felix2020federated, Hosseini2020FederatedLO} specifically solving such scenario. For our framework, one may concatenate some anomaly-detection models (e.g. auto-encoders) and collaboratively train a classifier for such scenario. As long as one can extract good features to classify a part of labels, our method can be applied to concatenate those good features to classify all labels. 

\subsection{Using a decoder to reconstruct}
When mentioning encoder, it is natural to ask if it helps to combine with a decoder to reconstruct. Especially for the label skew scenario, the network can only remember those information related to client's own labels. Can we retain some information by auto-encoder? 

We tried but we did not get better results in terms of final accuracy, and the convergence is even slowed down by the auto-encoder. According to information bottleneck theory \cite{Tishby2015DeepLA}, supervised learning forgets data information and only remembers those information with label, while unsupervised learning tries to remember data information as much as possible. Their goals are contradicted, so we get slow convergence. We record this failed attempt for the reference of other researchers. 


\subsection{IID data and model selection}
Our algorithm can bring more improvement when data is non-IID, while there is little improvement when data is IID. If label distribution is IID among clients, the models submitted by each cluster only bring similar features, thus concatenating them offers little help. In fact, \cite{li2021federated} shows that FedAvg is already good under IID data distribution setting. %Therefore our research focus is to solve the difficult label skew settings, where FedAvg and other FL algorithms have significant accuracy decay. 

Considering the IID scenario, a future research direction of this algorithm is to select the best cluster number $K$. %If $K$ is too large and similar clients are divided into different clusters, they may upload similar features which does not help. If we cluster them together, they can train better feature encoders based on more data. 
This is an adaptive model selection problem based on data distribution. 

Further, our method allows model selection flexibility among clusters. Each cluster does not have to train the same model. Clusters with powerful computing devices and more data can train heavier models for more rounds. Therefore, computing power and data quantity can also be taken into consideration during clustering.  

% \subsection{Other clustering methods}
% The current clustering method in FedConcat framework is simple, however clients need to share their label distribution information. If clients do not wish to leak label distribution, one can consider other clustering methods. However, they need extra computation or leak other feature information. 

% For example, IFCA \cite{Ghosh2020AnEF} allows clients to adaptively select cluster membership by minimum loss criterion, but it requires multiple times of communication cost and inference load. \cite{Briggs2020FederatedLW} needs many extra communication rounds to pre-train a decent model, and then it can perform clustering with uploaded gradient information. \cite{Rad2021FederatedLW} requires the centers of client's local data, which may leak some information of private data. 

% All clustering methods require some statistical information of clients. One can select methods according to different privacy protection requirements. Utilizing label distribution information is the simplest with low communication and computation cost, and our experimental results show its efficacy. And it does not leak any feature information. Therefore, we recommend this way if permitted. 

==> del/experiments.tex <==
\section{Experiments}
\label{sec:exp}

\change{We have conducted extensive experiments to evaluate our method. Through comprehensive experiments, we find that our techniques consistently outperform baseline methods, delivering superior accuracy and more stable convergence under various label skews. Importantly, our methods remain effective in scenarios characterized by partial client participation, large models, and an increased number of clients. The introduced label inference and clustering components are both straightforward and effective. Due to the space limit, we put the following experiments in Appendix.} 

\begin{itemize}
    \item D.2: training curves with communication costs.
    \item D.3: training curves with computation costs.
    \item D.4: compared to baselines on the concatenated model.
    \item D.5: varying the number of clusters.
    \item D.6: more results on varying the clustering strategies.
    \item D.7: client partial participation settings. 
    \item D.8: more results and analysis on large models.
    \item D.9: more results on varying the number of clients.
    \item D.10: analyzing FedConcat-ID label inference module.
\end{itemize}


\begin{table*}[ht]
\centering
\caption{Experimental results of our methods compared with baselines with same communication cost. The model of baseline algorithms is the model of one cluster in FedConcat. \YQ{We repeat experiments with three different random seeds.}}
\label{tbl:main}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c||c|c||c|}
\hline
Dataset & Partition & FedAvg & FedProx & MOON & FedRS & FedLC & FedConcat & FedConcat-ID & Centralized \\ \hline
\multirow{4}{*}{CIFAR-10} & $\#C=2$ & 53.6\%$\pm$0.8\% & 53.1\%$\pm$0.6\% & 53.4\%$\pm$1.3\% & 53.8\%$\pm$0.8\% & 49.8\%$\pm$0.6\% & \textbf{56.9\%$\pm$0.2\%}& \textbf{56.5\%$\pm$2.6\%} & \multirow{4}{*}{70.2\%$\pm$0.9\%} \\ \cline{2-9}
& $\#C=3$ & 57.6\%$\pm$0.6\% & 57.4\%$\pm$0.8\% & 58.6\%$\pm$1.8\% & 59.1\%$\pm$1.4\% & 58.1\%$\pm$1.4\% & \textbf{62.0\%$\pm$0.6\%}& \textbf{61.8\%$\pm$0.8\%}& \\ \cline{2-9}
& $p_k \sim Dir(0.1)$ & 53.0\%$\pm$1.0\% & 52.8\%$\pm$1.0\% & 53.1\%$\pm$3.5\% & 54.8\%$\pm$0.3\% & 53.7\%$\pm$0.8\% & \textbf{57.7\%$\pm$0.4\%}& \textbf{56.9\%$\pm$1.4\%}& \\ \cline{2-9}
& $p_k \sim Dir(0.5)$ & 59.9\%$\pm$0.5\% & 59.9\%$\pm$0.6\% & 61.2\%$\pm$1.8\% & 61.5\%$\pm$0.8\% & 61.5\%$\pm$1.1\% & \textbf{64.2\%$\pm$0.7\%}& \textbf{63.7\%$\pm$0.8\%}& \\ \hline
\multirow{4}{*}{SVHN} & $\#C=2$ & 82.8\%$\pm$0.5\% & 82.6\%$\pm$0.6\% & 83.0\%$\pm$0.1\% & 79.5\%$\pm$1.2\% & 75.7\%$\pm$2.3\% & \textbf{83.4\%$\pm$1.4\%}& \textbf{83.2\%$\pm$1.9\%}& \multirow{4}{*}{86.2\%$\pm$0.9\%}  \\ \cline{2-9}
& $\#C=3$ & 85.2\%$\pm$0.4\% & 85.2\%$\pm$0.6\% & 84.7\%$\pm$0.4\% & 85.7\%$\pm$0.4\% & 84.8\%$\pm$0.4\% & \textbf{86.0\%$\pm$0.9\%}& \textbf{86.1\%$\pm$0.5\%}& \\ \cline{2-9}
& $p_k \sim Dir(0.1)$ & \textbf{84.0\%$\pm$1.3\%} & 83.9\%$\pm$1.2\% & 83.7\%$\pm$1.1\% & 80.9\%$\pm$0.9\% & 78.8\%$\pm$0.8\% & 83.2\%$\pm$0.9\%& 82.9\%$\pm$0.3\% & \\ \cline{2-9}
& $p_k \sim Dir(0.5)$ & 87.2\%$\pm$0.2\% & 87.2\%$\pm$0.2\% & 87.2\%$\pm$0.2\% & 87.1\%$\pm$0.1\% & 87.1\%$\pm$0.5\% & \textbf{87.5\%$\pm$0.1\%}& \textbf{87.9\%$\pm$0.3\%}& \\ \hline
\multirow{4}{*}{FMNIST} & $\#C=2$ & 79.0\%$\pm$4.7\% & 81.8\%$\pm$2.8\% & 81.4\%$\pm$1.4\% & 78.3\%$\pm$1.8\% & 77.7\%$\pm$2.9\% & \textbf{84.4\%$\pm$0.6\%}& \textbf{83.0\%$\pm$2.0\%}& \multirow{4}{*}{88.4\%$\pm$0.2\%} \\ \cline{2-9}
& $\#C=3$ & 84.7\%$\pm$1.4\% & 85.7\%$\pm$0.3\% & 84.6\%$\pm$1.9\% & 85.8\%$\pm$0.8\% & 86.0\%$\pm$0.3\% & \textbf{87.1\%$\pm$0.2\%}& \textbf{86.6\%$\pm$0.1\%}& \\ \cline{2-9}
& $p_k \sim Dir(0.1)$ & 85.1\%$\pm$0.5\% & \textbf{85.2\%$\pm$0.8\%} & 85.0\%$\pm$0.1\% & 82.5\%$\pm$0.5\% & 82.1\%$\pm$1.6\% & 84.5\%$\pm$0.1\%& 85.0\%$\pm$0.4\% & \\ \cline{2-9}
& $p_k \sim Dir(0.5)$ & 87.5\%$\pm$0.3\% & 87.4\%$\pm$0.4\% & 87.4\%$\pm$0.5\% & 87.5\%$\pm$0.5\% & 87.5\%$\pm$0.4\% & \textbf{87.7\%$\pm$0.1\%}& \textbf{87.5\%$\pm$0.2\%}& \\ \hline
\end{tabular}
 }
% \vspace{-10pt}
\end{table*}

\subsection{Experiment Setups}
\paragraph{Datasets} 
% According to a popular benchmark study \cite{li2021federated}, CIFAR-10 dataset is the most difficult and has much accuracy degradation under non-IID partition. Therefore we mainly experiment on CIFAR-10 dataset. 
\change{Our experiments engage CIFAR-10 \citep{krizhevsky2009learning}, FMNIST \citep{xiao2017fashion}, SVHN \citep{netzer2011reading}, CIFAR-100 \citep{krizhevsky2009learning}, and Tiny-ImageNet datasets \citep{wu2017tiny} to evaluate our algorithm. The partition strategy from \citet{li2021federated} generates various non-IID settings, with a focus on label skews, given their significant accuracy degradation \cite{li2021federated}. In experiments, $\#C=k$ represents clients with $k$ unique labels, while $p_k \sim Dir(\beta)$ denotes the Dirichlet distribution sampled proportion of each class samples assigned to each client. By default, we divide whole dataset into 40 clients.}

\paragraph{Baselines}
\change{Our method is compared with well-known, open-sourced FL methods including FedAvg \cite{mcmahan2016communication}, FedProx \cite{lifedprox}, MOON \cite{li2021model}, FedRS \cite{li2021fedrs}, and FedLC \cite{zhang2022federated} which cater to label skews. The baseline settings replicate those from \citet{li2021federated}, running 50 rounds with each client training 10 local epochs per round, batch size 64, and learning rate 0.01 using SGD optimizer with weight decay $10^{-5}$.}

\paragraph{Models}
\change{To investigate diverse scenarios with different clients' capacities, we experiment with three different neural networks: simple CNN, VGG-9, and ResNet-50. By default, we use simple CNN. Appendix D.1 provides more details on the setups.}


 % in Appendix \ref{sec:more_curve} and computation cost in \ref{sec:anal_computation}. We experiment with baseline algorithms on concatenated models in Appendix \ref{sec:more_concatenated_model}, varying the number of clusters in Appendix \ref{sec:exp_num_cluster}, FL clustering strategies in Appendix \ref{sec:exp_cluster_FL}, partial participation in Appendix \ref{sec:exp_partial}, heavy model in Appendix \ref{sec:exp_resnet} and scalability in Appendix \ref{sec:more_scalab}. We analyze the label inference and training curves of FedConcat-ID in Appendix \ref{sec:more_exp_concat_id}.

% Initially we try to run a full epoch, but the global classifier has trouble converging under quantity-based label skew partition. We think it is because linear classifier is easy to converge locally, so we need to reduce its local steps to make it converge globally. Experimental results show that 3 local steps is a good choice, so this is our default setting for all experiments in this work. 



\subsection{Effectiveness}
\label{sec:main_exp}
% Here we divide whole dataset into 40 clients using the same partition strategy in \cite{li2021federated}, and set the number of clusters $K=5$. We choose $K=5$ because it is stable and achieves relatively good accuracy in various settings, as is shown in the supplementary material. Small $K$ has similar accuracy to FedAvg, while large $K$ can lead to unstable convergence under some cases. 

\change{We evaluate the performance of FedConcat and FedConcat-ID against other baselines. By default, our configuration includes a division of the 40 clients into $K=5$ clusters, and 200 rounds allocated for training the classifier. In order to equate the communication cost of FedConcat to that of 50 rounds of FedAvg, we set the encoder training to 31 rounds. For the FMNIST dataset, due to its image size differing from CIFAR-10 and SVHN, we record the test accuracy at classifier round 173 to maintain similar communication costs. } 

\change{The results in Table \ref{tbl:main} illustrate that FedConcat consistently outperforms the other five FL algorithms in most scenarios. Specifically, in the challenging CIFAR-10 dataset, both FedConcat and FedConcat-ID offer an average improvement of about 4\%. When considering partition types, notable improvements are evident in the more complex $\#C=2$ and $\#C=3$ partitions. For the Dirichlet-based label distributions of SVHN and FMNIST datasets, since the label skews are slight, the accuracy degradation of baseline algorithms from centralized training (200 epochs) is small. In such scenarios, our methods exhibit comparable accuracy with the baselines.}
% we fix 200 classifier communication rounds and calculate that we can train encoder for 31 communication rounds. Since FMNIST has different input data dimension and model structure, there can only be 31 encoder rounds with 173 classifier rounds. 

% However, we find that $\mu \in \{1,5\}$ of MOON is good for CIFAR-10 dataset but not good for SVHN and FMNIST. Therefore we further try smaller $\mu \in \{0.001,0.01,0.1\}$ of MOON and find that generally $\mu=0.001$ is good for SVHN and FMNIST. 


% Under Dirichlet distribution based label skew of FMNIST, it cannot beat state-of-the-art MOON algorithm, but its accuracy is still very close. 




% We can conclude that FedConcat achieves better and more stable global model accuracy with smaller communication and computation cost. 
% We can set the number of rounds for training the encoder as the number of communication rounds that FedAvg becomes converged. 

\subsection{Scalability}
\label{sec:scalab}
\change{In this section, we evaluate the scalability of FedConcat. We keep the number of clusters $K=5$. During each round, a random selection of 50\% of the clients is sampled to participate in FL training. The results, as illustrated in Table \ref{tbl:scala_main}, confirm that both FedConcat and FedConcat-ID continue to outperform baseline algorithms with 100 or 200 clients and partial participation settings. }

\begin{table}[ht]
\centering
\caption{Scalability of FedConcat and FedConcat-ID compared with baselines on CIFAR-10 dataset. }
\label{tbl:scala_main}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c||c|c|}
\hline
\#Clients & {Partition} & {FedAvg} & {FedProx} & {MOON} & {FedRS} & {FedLC} & {FedConcat} & {FedConcat-ID} \\ \hline
\multirow{4}{*}{100} & $\#C=2$ & 44.4\% & 43.7\% & 44.4\% & \textbf{54.4\%} & 52.6\% & 51.0\% & 53.2\% \\ \cline{2-9}
& $\#C=3$ & 55.4\% & 54.6\% & 55.2\% & 56.5\% & 54.8\% & \textbf{59.0\%}& \textbf{59.3\%} \\ \cline{2-9}
& $p_k \sim Dir(0.1)$ & 45.0\% & 44.8\% & 45.3\% & 50.5\% & 50.0\% & 49.1\%& \textbf{50.7\%} \\ \cline{2-9}
& $p_k \sim Dir(0.5)$ & 58.1\% & 58.3\% & 57.7\% & 59.0\% & 58.1\% & \textbf{63.3\%}& \textbf{62.2\%}  \\ \hline


\multirow{4}{*}{200} & $\#C=2$ & 39.7\% & 40.9\% & 40.3\% & 46.2\% & 48.6\% & \textbf{48.9\%} & 44.6\%  \\ \cline{2-9}
& $\#C=3$ & 47.7\% & 48.2\% & 47.8\% & 51.5\% & 51.0\% & \textbf{53.1\%}& \textbf{51.8\%} \\ \cline{2-9}
& $p_k \sim Dir(0.1)$ & 40.5\% & 41.2\% & 40.9\% & 43.6\% & 43.7\% & \textbf{47.6\%}& \textbf{46.7\%}  \\ \cline{2-9}
& $p_k \sim Dir(0.5)$ & 53.9\% & 53.5\% & 53.9\% & 54.4\% & 53.7\% & \textbf{56.7\%}& \textbf{56.8\%}  \\ \hline

\end{tabular}
 }
% \vspace{-10pt}
\end{table}



\subsection{Experiments on Larger Model}


\begin{table*}[ht]
\centering
\caption{Experimental results on CIFAR-100 and Tiny-ImageNet with ResNet-50. We tune the weight decay among $\{0.00001,0.001,0.002,0.005\}$ for all algorithms. We present the average and standard deviation of the last 10 rounds.}
\label{tbl:resnet}

\resizebox{2\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c||c|c||c|}
\hline
Dataset & Partition & FedAvg & FedProx & MOON & FedRS & FedLC & FedConcat & FedConcat-ID & Centralized \\ \hline
\multirow{4}{*}{CIFAR-100} & $\#C=2$ & 8.4\%$\pm$1.2\% & 8.1\%$\pm$1.3\% & 8.0\%$\pm$1.0\% & 7.0\%$\pm$1.5\% & 3.8\%$\pm$0.4\%  & \textbf{18.5\%$\pm$0.7\%} & \textbf{16.4\%$\pm$0.8\%} & \multirow{4}{*}{70.5\%$\pm$0.1\%} \\ \cline{2-9}
& $\#C=3$ & 21.6\%$\pm$2.8\% & 18.7\%$\pm$6.0\% & 19.0\%$\pm$2.4\% & 19.2\%$\pm$1.7\% & 12.6\%$\pm$0.7\% & \textbf{34.4\%$\pm$1.1\%} & \textbf{32.9\%$\pm$0.6\%} &  \\ \cline{2-9}
& $p_k \sim Dir(0.1)$ & 52.4\%$\pm$4.9\% & 51.5\%$\pm$8.1\% & 55.2\%$\pm$3.3\% & 51.8\%$\pm$2.8\% & 50.5\%$\pm$2.9\% & \textbf{61.2\%$\pm$0.4\%} & \textbf{62.1\%$\pm$0.5\%} &  \\ \cline{2-9}
& $p_k \sim Dir(0.5)$ & 62.0\%$\pm$1.2\% & 61.2\%$\pm$1.3\% & 61.9\%$\pm$0.9\% & 61.9\%$\pm$1.2\% & 61.4\%$\pm$1.3\% & \textbf{66.3\%$\pm$0.1\%} & \textbf{65.6\%$\pm$0.1\%} &  \\ \hline

\multirow{4}{*}{Tiny-ImageNet} &  $\#C=2$ & 3.1\%$\pm$0.4\% & 2.7\%$\pm$0.3\% & 3.0\%$\pm$0.4\% & 3.1\%$\pm$0.1\% & 2.0\%$\pm$0.1\%  & \textbf{4.3\%$\pm$0.1\%} & \textbf{4.3\%$\pm$0.2\%} & \multirow{4}{*}{49.9\%$\pm$0.2\%}    \\ \cline{2-9}
& $\#C=3$ & 4.9\%$\pm$2.4\% & 5.1\%$\pm$1.0\% & 6.3\%$\pm$1.7\% & 3.3\%$\pm$0.4\% & 1.7\%$\pm$0.1\%  & \textbf{11.7\%$\pm$0.3\%} & \textbf{9.6\%$\pm$0.2\%} &  \\ \cline{2-9}
& $p_k \sim Dir(0.1)$ & 40.8\%$\pm$0.5\% & 40.8\%$\pm$0.6\% &  40.6\%$\pm$0.8\% & 39.7\%$\pm$0.7\% & 39.9\%$\pm$0.8\%  & \textbf{43.1\%$\pm$0.2\%} & \textbf{42.6\%$\pm$0.2\%} &  \\ \cline{2-9}
& $p_k \sim Dir(0.5)$ & 44.0\%$\pm$0.6\% & 44.2\%$\pm$0.7\% &  44.1\%$\pm$0.5\% & 43.6\%$\pm$0.9\% & 43.9\%$\pm$0.5\%  & \textbf{44.3\%$\pm$0.1\%} & 43.8\%$\pm$0.2\% &   \\ \hline


\end{tabular}
 }

% \resizebox{1\columnwidth}{!}{
% % \begin{tabular}{|c|c|c|c|c|c||c|c|}
% % \hline
% % Partition & FedAvg & FedProx & MOON & FedRS & FedLC & FedConcat & FedConcat-ID  \\ \hline
% % $\#C=2$ & 8.4\%$\pm$1.2\% & 8.1\%$\pm$1.3\% & 7.2\%$\pm$0.9\% & 7.0\%$\pm$1.5\% & 3.8\%$\pm$0.4\% & \textbf{12.1\%$\pm$0.2\%} & \textbf{12.0\%$\pm$0.4\%} \\ \hline
% % $\#C=3$ & 21.6\%$\pm$2.8\% & 18.7\%$\pm$6.0\% & 20.0\%$\pm$2.7\% & 19.2\%$\pm$1.7\% & 12.6\%$\pm$0.7\% & \textbf{26.7\%$\pm$0.2\%} & \textbf{24.6\%$\pm$0.2\%} \\ \hline

% % $p_k \sim Dir(0.1)$ & 52.4\%$\pm$4.9\% & 51.5\%$\pm$8.1\% & 48.8\%$\pm$0.7\% & 51.8\%$\pm$2.8\% & 50.5\%$\pm$2.9\% & \textbf{53.6\%$\pm$0.1\%} & \textbf{56.4\%$\pm$0.1\%} \\ \hline
% % $p_k \sim Dir(0.5)$ & 57.0\%$\pm$0.8\% & 58.2\%$\pm$2.5\% & 49.7\%$\pm$1.1\% & 57.1\%$\pm$1.8\% & 57.7\%$\pm$1.9\% & \textbf{59.5\%$\pm$0.0\%} & \textbf{59.8\%$\pm$0.0\%} \\ \hline

% % \end{tabular}
% \begin{tabular}{c|c|c|c|c}
% \hline
% Algorithm & $\#C=2$ & $\#C=3$ & $p_k \sim Dir(0.1)$ & $p_k \sim Dir(0.5)$ \\ \hline
% FedAvg & 8.4\%$\pm$1.2\% & 21.6\%$\pm$2.8\% & 52.4\%$\pm$4.9\% & 57.0\%$\pm$0.8\% \\ 
% FedProx & 8.1\%$\pm$1.3\% & 18.7\%$\pm$6.0\% & 51.5\%$\pm$8.1\% & 58.2\%$\pm$2.5\% \\ 
% MOON & 7.2\%$\pm$0.9\% & 20.0\%$\pm$2.7\% & 48.8\%$\pm$0.7\% & 49.7\%$\pm$1.1\% \\ 
% FedRS & 7.0\%$\pm$1.5\% & 19.2\%$\pm$1.7\% & 51.8\%$\pm$2.8\% & 57.1\%$\pm$1.8\% \\ 
% FedLC & 3.8\%$\pm$0.4\% & 12.6\%$\pm$0.7\% & 50.5\%$\pm$2.9\% & 57.7\%$\pm$1.9\% \\ \hline
% FedConcat & \textbf{12.1\%$\pm$0.2\%} & \textbf{26.7\%$\pm$0.2\%} & \textbf{53.6\%$\pm$0.1\%} & \textbf{59.5\%$\pm$0.0\%} \\ 
% FedConcat-ID & \textbf{12.0\%$\pm$0.4\%} & \textbf{24.6\%$\pm$0.2\%} & \textbf{56.4\%$\pm$0.1\%} & \textbf{59.8\%$\pm$0.0\%} \\ \hline
% Centralized & \multicolumn{4}{c}{0} \\
% \hline
% \end{tabular}

%  }
% \vspace{-10pt}
\end{table*}

% Since simple CNN has limited representation power and underfits CIFAR-10 dataset, we try heavier VGG-9 and ResNet-50 \cite{he2016deep}, which has better accuracy in CIFAR-10. However, when training ResNet-50 using FedAvg, the training curve is very unstable. The accuracy jumps back and forth from 20\% to 80\%. Such instability is also shown in \cite{li2021federated}. Therefore we only show experimental results of VGG-9 in Figure \ref{fig:heavy}, which has more stable convergence.

% Actually compared with simple CNN, VGG-9 also has fluctuating training curve. Heavy model is more difficult to train, and may be worse in non-IID FL setting. For one thing, heavier models are over-parameterized, so there are many possible optimization directions to achieve local convergence. When it comes to aggregation, averaging these optimization directions can possibly lead to a bad global model. For another, the batch normalization layer in ResNet-50 may not work by simply averaging each clients' parameters. 

% To investigate the influence of the model architecture on the FL approaches, we compare FedConcat and FedConcat-ID with the other baselines with VGG-9 on CIFAR-10. The results are shown in Figure \ref{fig:heavy}.
% Similarly, our FedConcat still has significant advantage on VGG-9 model for the extreme non-IID $\#C=2$ case. It can achieve higher accuracy with smooth convergence. FedConcat-ID achieves slightly lower accuracy than FedConcat, but can still outperform five baseline algorithms. 


\change{In this section, we conduct experiments on larger models, more clients and more complicated tasks, i.e. training ResNet-50 on CIFAR-100 and Tiny-ImageNet. There are 200 clients, and in each round a random selection of 20\% of the clients participate in the training. For baseline algorithms, we train 500 communication rounds. For FedConcat and FedConcat-ID, we train 480 encoder rounds and 500 classifier rounds to match the communication cost. Since ResNet-50 has huge memory and computation overhead, we set the number of clusters as 2 to constrain memory and computation costs. }


\change{New problems arise when training FedConcat with ResNet-50 on CIFAR-100 and Tiny-ImageNet. Firstly, local cluster models tend to overfit since each local cluster witnesses fewer data compared with training on all clients. Secondly, the cluster sizes become quite unbalanced since the label distribution points become more sparse in the high dimensional (100-D or 200-D) space. Some points may be so far from others that they are allocated into a very small cluster. Thirdly, the training process of the final classifier layer is more difficult to converge since there are many more hidden neurons in ResNet-50 than simple CNN. }

\change{To address these problems, we increase the weight decay factor to tackle overfitting. Client members of the majority cluster are relocated to force each cluster to be balanced. At the beginning of the post-training stage, the global classifier is initialized with parameters of cluster classifiers to speed up convergence. We discuss these adaptations in detail and conduct ablation studies in Appendix D.8. }

\change{As shown in Table \ref{tbl:resnet}, by tackling these issues, our methods achieve higher accuracy than baselines by an average of 8\% on CIFAR-100 and 2\% on Tiny-ImageNet.}% The tuning of weight decay is to address the overfitting problem, which is further analyzed in Appendix \ref{sec:exp_resnet}. }


\subsection{Effect of Clustering}
\label{sec:large-model}
If we concatenate all models from all clients without clustering, when there are a large number of clients, our global model can become very large. Large final model leads to heavy communication cost when training the global classifier. During inference, it also costs much computation time. Moreover, concatenating all models from all clients can suffer from unstable convergence and low test accuracy, since each client can have limited training samples. 

An experiment on CIFAR-10 is illustrated in Figure \ref{fig:wcluster}, where we show the test accuracy at each classifier round after training 100 encoder rounds. No clustering means each client trains a model for server to concatenate, where each client model is only trained with few samples and prone to overfit. Since those models are not well-trained, concatenating their encoders can hardly extract good features. From Figure \ref{fig:wcluster}, we can observe that clustering not only reduces communication cost, but also effectively improves model quality with more samples. 

\begin{figure}[ht]
    \centering
    % \vspace{-10pt}
    \includegraphics[width=0.9\columnwidth]{figures/wcluster-new.pdf}
    % \vspace{-10pt}
    \caption{Training curves with clustering versus without clustering on CIFAR-10 (40 clients). }
    \label{fig:wcluster}
\end{figure}

FedConcat concatenates a cluster of models into a large model. If we directly train such a large model with other FL algorithms, does FedConcat still have advantage? 
To answer this question, we train baseline algorithms on the model with equivalent size to the final concatenated model of FedConcat. The training curves on CIFAR-10 dataset are shown in Figure \ref{fig:large}, which illustates that FedConcat still keeps its advantage when compared with the concatenated model. 


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/large-label2-new.pdf}
    % fig: 200 comm rounds
    %\subfloat[\#C=2]{\includegraphics[width=0.4\textwidth]{figures/large-label2.pdf}}
    \ \ \ \ \ 
    %\subfloat[$p_k \sim Dir(0.5)$]{\includegraphics[width=0.4\textwidth]{figures/large-dir.pdf}}
    % \vspace{-10pt}
    \caption{Comparing with baselines on the final global model of FedConcat on CIFAR-10 (40 clients, $\#C=2$).}
    \label{fig:large}
    % \vspace{-10pt}
\end{figure}

\subsection{Comparing with Other Clustered FL}
\label{sec:main_cfl}
\change{In this section, we employ other clustered FL algorithms during our clustering stage. We conduct experiments with three clustering-based methods including IFCA \cite{Ghosh2020AnEF}, recently proposed FedSoft \cite{ruan2022fedsoft} and FeSEM \cite{long2023multi}. We adhere to the same experimental settings as specified in Section \ref{sec:main_exp}. The results for the CIFAR-10 dataset are presented in Table \ref{tbl:cfl}. It can be observed that both FedConcat and FedConcat-ID outperform other clustering strategies. FeSEM incorporates an additional proximal loss term during local training, which results in an extra computational burden similar to FedProx. Both IFCA and FedSoft entail multiple instances of communication cost as all cluster models are transferred to clients in each round. Thus, the clustering strategies of FedConcat and FedConcat-ID prove to be both effective and efficient. }

\begin{table}[htbp]
\centering
\caption{Experimental results of FedConcat and FedConcat-ID compared with other clustering strategies on CIFAR-10.}
\label{tbl:cfl}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c||c|c|}
\hline
Partition & IFCA & FedSoft & FeSEM & FedConcat & FedConcat-ID \\ \hline
$\#C=2$ & 54.5\%$\pm$0.9\% & 49.5\%$\pm$0.6\% & 54.0\%$\pm$1.5\% & \textbf{56.9\%$\pm$0.2\%}& \textbf{56.5\%$\pm$2.6\%} \\ \hline
$\#C=3$ & 60.0\%$\pm$0.9\%  & 56.1\%$\pm$0.9\% & 60.4\%$\pm$2.4\% & \textbf{62.0\%$\pm$0.6\%}& \textbf{61.8\%$\pm$0.8\%} \\ \hline
$p_k \sim Dir(0.1)$ & 49.5\%$\pm$5.7\%  & 51.8\%$\pm$1.2\% & 56.1\%$\pm$1.7\% & \textbf{57.7\%$\pm$0.4\%}& \textbf{56.9\%$\pm$1.4\%} \\ \hline
$p_k \sim Dir(0.5)$ & 63.3\%$\pm$0.2\% & 59.5\%$\pm$1.5\% & 63.1\%$\pm$0.8\% & \textbf{64.2\%$\pm$0.7\%}& \textbf{63.7\%$\pm$0.8\%} \\ \hline
\end{tabular}
 }
% \vspace{-10pt}
\end{table}


% To solve these problems, we propose to cluster clients to a limited number of groups. Clustering not only lowers communication cost, but also strengthens model quality with more samples. 




% \subsection{Results without clustering}
% In this section, we test whether the aggregation idea works. We divide CIFAR-10 dataset into 10 clients. For the benchmark \cite{li2021federated}, the server performs 50 communication rounds and each client trains 10 local epochs per round. 

% For our new algorithm, each client trains a well-fitted model and server concatenates those 10 encoders to train a global classifier. We set each client to train 200 local epochs. The global classifier is trained 200 communication rounds. \YQ{We run three times for FedConcat and report the mean accuracy and standard derivation. }

% \begin{table}[h]
% \centering
% \caption{Experimental results of FedConcat on CIFAR-10. }

% \label{tbl:simple}
% \resizebox{1\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Partition & FedConcat & FedAvg & FedProx & SCAFFOLD & FedNova \\ \hline
% $\#C=2$ & \textbf{61.2\%$\pm$1.5\%} & 49.8\%$\pm$3.3\% & 50.7\%$\pm$1.7\% & 49.1\%$\pm$1.7\% &46.5\%$\pm$3.5\% \\ \hline
% $\#C=3$ & \textbf{67.7\%$\pm$1.3\%} & 58.3\%$\pm$1.2\% & 57.1\%$\pm$1.2\% & 57.8\%$\pm$1.4\% &54.4\%$\pm$1.1\% \\ \hline
% $p_k \sim Dir(0.5)$ & 69.5\%$\pm$0.2\% & 68.2\%$\pm$0.7\% & 67.9\%$\pm$0.7\% & \textbf{69.8\%$\pm$0.7\%}& 66.8\%$\pm$1.5\% \\ \hline
% %$q \sim Dir(0.5)$ & 70.6\% & \textbf{72.0\%} \\ \hline
% %$\hat{\mb{x}} \sim Gau(0.1)$ & 67.6\% & \textbf{70.1\%} \\ \hline
% \end{tabular}
% }
% % \vspace{-20pt}
% \end{table}

% Results are shown in Table \ref{tbl:simple}. As we can see, FedConcat can achieve a significant improvement than the best benchmark results (among FedAvg, FedProx, SCAFFOLD and FedNova) under quantity-based label skew scenario.  

% What's more, FedConcat needs much less computation and communication cost to achieve such accuracy in this experiment. According to our calculation, compared with FedAvg, the communication cost of FedConcat is about 70\%, the computation cost in client side is about 44\% and the computation cost in server side is about 60\%. 


% \subsection{Baselines running on the concatenated model}
% \label{sec:large-model}
% FedConcat concatenates a cluster of models and leads to a large model. If we directly train such a large model with other FL algorithms, does FedConcat still have advantage? 
% In this section, baseline algorithms are trained on the model with equivalent size to the final concatenated model of FedConcat. The training curves on CIFAR-10 dataset are shown in Figure \ref{fig:large}, which illustates that FedConcat still keeps its advantage when compared with the concatenated model. \change{More results are listed in Appendix \ref{sec:more_concatenated_model}. }


% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=1\columnwidth]{figures/large-label2-new.pdf}
%     % fig: 200 comm rounds
%     %\subfloat[\#C=2]{\includegraphics[width=0.4\textwidth]{figures/large-label2.pdf}}
%     \ \ \ \ \ 
%     %\subfloat[$p_k \sim Dir(0.5)$]{\includegraphics[width=0.4\textwidth]{figures/large-dir.pdf}}
%     \vspace{-10pt}
%     \caption{The training curves on CIFAR-10 dataset. Baseline algorithms are trained on model with same size to final global model of FedConcat. The data partition is $\#C=2$.}
%     \label{fig:large}
%     \vspace{-10pt}
% \end{figure}

%In summary, when compared with the concatenated model, FedConcat still keeps its advantage on $\#C=2$ partition. %However, under $p_k \sim Dir(0.5)$ distribution, its convergence accuracy cannot reach that high, but is still comparable. This shows that FedConcat can alleviate the accuracy loss in extreme non-IID cases. In relatively IID settings, FedAvg is already a good solution. And both cases show that FedConcat can achieve comparable accuracy with much lower communication cost. 





% \begin{figure}[!]
%     \centering
%     \includegraphics[width=1\columnwidth]{figures/heavy-label2-new.pdf}
%     \caption{The training curves on CIFAR-10 dataset with VGG-9. The data partition is $\#C=2$.}
%     \label{fig:heavy}
% \end{figure}




==> del/introduction.tex <==
\section{Introduction}
\label{sec:intro}
A good machine learning model usually needs a large high-quality dataset to train. However, due to privacy concern and regulations such as GDPR \cite{voigt2017eu}, sometimes it is not allowed to collect original data for centralized training. Federated learning (FL) \cite{kairouz2019advances,li2019flsurvey,litian2019survey,yang2019federated} is proposed to let data owners collaboratively train a better machine learning model without exposing raw data. It has become a hot research topic \cite{li2020practical,dai2020federated,he2020group,lifedprox,karimireddy2019scaffold,liu2020secure,wu2020privacy}. FL has many potential practical applications~\cite{bonawitz2019towards,hard2018federated,kaissis2020secure}. For example, different hospitals can collectively train a FL model for diagnosing diseases through medical imaging, while protecting the privacy of individual patients. 

A typical framework of FL is FedAvg \cite{mcmahan2016communication}, where the clients train and send their local models to the server, and the server averages the local models to update the global model in each round. It has been shown that data heterogeneity is a challenging problem in FL, since non-IID data distributions among FL clients can degrade the FL model performance and slow down model convergence \cite{karimireddy2019scaffold,Li2020On,hsu2019measuring, li2021federated}. According to \citet{li2021federated}, non-IID data includes label skews, feature skews and quantity skews. In this paper, we focus on label skews (i.e., the label distributions of different clients are different), which is popular in reality (e.g., disease distributions vary across different areas). 

Researchers have put some promising effort to address the above label skew challenge. For example, FedProx \cite{lifedprox} uses the $L_2$ distance between the local model and the global model to regularize the local training. MOON \cite{li2021model} regularizes the local training using the similarity between representations of the local model and the global model.  FedRS \cite{li2021fedrs} restricts the updates of unseen classes during local training. FedLC \cite{zhang2022federated} further calibrates logits to reduce the updates of minority classes. 
% \YQ{In this paper, we focus on label skews, where each client only has relatively large number of samples of several classes but fewer or no data of many other classes.} According to the previous benchmark study \cite{li2021federated}, label skews are the most challenging with largest accuracy degradation, and none of the four FL algorithms studied (FedAvg \cite{mcmahan2016communication}, FedProx \cite{lifedprox}, SCAFFOLD \cite{karimireddy2019scaffold} and FedNova \cite{wang2020tackling}) can consistently outperform the others in all settings.
\YQ{The key idea of existing studies is usually to reduce the drift produced in local training \cite{lifedprox,li2021model,karimireddy2019scaffold, li2021fedrs, zhang2022federated} or design a better federated averaging scheme in the server \cite{wang2020tackling, Wang2020Federated}. Those algorithms are based on the averaging framework.} They attempt to address the label skew problem by mitigating its side effect in federated averaging. However, existing methods cannot achieve satisfactory performance. In label skews, the averaging methods may not make much sense, as each party may have very different models to predict different classes. \rev{Especially under extreme label skews where each client has quite different classes (e.g., face recognition), since the local optima are far from each other, averaging these local models leads to significant accuracy degradation. Even worse, it is challenging to quantify how label skews influence the model due to the diversity of label skews in practice. }
% Under non-IID settings, the global model can deviate from global optima, so these four algorithms still have a large accuracy gap in non-IID settings compared with the IID setting. Such a gap is more significant under label skew cases \cite{li2021federated}. Thus, label skews have been largely overlooked in previous FL studies.

% Rethinking the challenges of label skews, we ask this question: \textit{instead of performing federated averaging under label skews, can we treat label skews as a feature to exploit?} 
\change{In this paper, we think out of the model-averaging scheme, and propose to use model concatenation as the aggregation method.} Since each local model is good at classifying samples of several classes due to label skews, we propose to concatenate the features learned by the local models to combine the knowledge from the local models.
% Here, each model is an expert for classifying samples among its cluster. Instead of averaging, we use all features extracted by those models for prediction. 
For example, in the label skew setting, one client has sufficient data on cats with little data on dogs, while another client has sufficient data on dogs with little data on cats. Then, each client can train a local model which is good at predicting one class. Intuitively, concatenating those models can gather all key information, which can help train a good classifier for all classes among clients. This seemingly simple idea fundamentally changes the way of existing methods regarding label skews as an issue to avoid or mitigate. 

With this idea, we propose a novel FL algorithm to address label skews named FedConcat. First, the server divides clients into a few different clusters according to their label distributions. To address the privacy concern of uploading label distribution information, we develop an effective method to infer label distribution directly from the model. Second, FedAvg is conducted among each cluster to learn a good model for each kind of label distribution. Third, the server concatenates encoders of models of all clusters (i.e. neural networks except the last layer). Finally, with the parameters of the concatenated encoders fixed, the server and the clients jointly train a classifier on top of it using FedAvg. \change{We theoretically justify that concatenation keeps richer mutual information than averaging in the feature space by applying the information bottleneck theory. }

\rev{Among each cluster, clients have similar label distributions. The label skew problem is alleviated inside the cluster, so FedAvg is competent to train a good model for each cluster with slight label skews. Since the concatenated encoders have already extracted good features, the task of training a linear classifier in the final stage becomes simpler. Therefore, FedAvg can achieve good accuracy for the simplified task. Moreover, through clustering, we can control the size of global model by adjusting the number of clusters.} 

We conduct extensive experiments with various label skew settings. Our experimental results show that FedConcat can significantly improve the accuracy compared with the other state-of-the-art FL algorithms including FedAvg \cite{mcmahan2016communication}, FedProx \cite{lifedprox}, MOON \cite{li2021model}, FedRS \cite{li2021fedrs} and FedLC \cite{zhang2022federated}. \rev{The improvement is more significant under extreme label skews. Besides, FedConcat can achieve better accuracy with much smaller communication and computation costs compared with baselines.} %Therefore, FedConcat brings more benefits than previous FL algorithms to cross-device settings, where the label skews are severe and the commextractedon and computation costs are limited.

\rev{Our contributions can be summarized as follow:}
\begin{itemize}
    \item Instead of averaging, we propose a new aggregation method in FL by concatenating the local models. Moreover, we apply clustering technique to alleviate label skew and control the size of global model.
    \item We theoretically show that concatenation preserves more information than averaging from the information bottleneck perspective, which guarantees the effectiveness of our approach.
    \item We conduct extensive experiments to show the effectiveness and communication efficiency of FedConcat. Under various label skew settings of a popular FL benchmark \cite{li2021federated}, FedConcat can outperform baselines averagely by 4\% on CIFAR-10, by 8\% on CIFAR-100, by 2\% on Tiny-ImageNet, and by 1\% on FMNIST and SVHN datasets.
\end{itemize}

% \YQ{Moreover, our framework can be easily combined with the other state-of-the-art FL methods to further improve the performance.} %\YQ{Given the same communication cost, FedConcat can outperform these FL algorithms by at least 1\% global model test accuracy in most label skew cases.} %And our method can save much communication cost. 

\section{Background and Related Work}
% Non-IID data distribution is prevalent among different clients. For example, a certain disease may be common in one country, but rare in another country.

Denote $D^i=(X^i,Y^i)$ the local dataset of client $i$. Label skews mean that $P(Y^i)$ differs among clients. According to \citet{li2021federated}, label skews can lead to significant accuracy degradation of the global model. It is also prevalent in real-world scenarios. For example, the disease distributions differ in different regions, which leads to label skews when training a global automatic disease diagnosis system. 

Previous studies like FedAvg \cite{mcmahan2016communication} average all models submitted by clients. However, under the non-IID data distribution cases, each client trains a good local model towards its local optimum. While the local optima may be far from each other, simply averaging the local models may produce a global model that is also far from the global optimum. There are many existing studies aiming to solve the non-IID data distribution problem based on FedAvg \cite{mcmahan2016communication}. %Existing studies usually improve FedAvg by improving the local training stage, improving the model averaging stage, improving the data quality, and improving client selection.
% The accuracy decay of label skew can be explained by information bottleneck theory \cite{Tishby2015DeepLA}. It states that deep neural networks try to extract only information of raw data related to its label, and forget everything else. Therefore, in the case of label skew scenarios, the models can only extract information which can classify its own labels. Averaging parameters generally costs many communication rounds to converge on label skew scenario. 

% \section{Related Work}
% \subsection{Non-IID in FL}

%\paragraph{Improving Local Training.} 
\rev{A popular way is to improve local training so that the local model is not too far from the global optimum. For example,} FedProx \cite{lifedprox} adds a regularization term which measures the distance between the local model and the global model. MOON \cite{li2021model} shares a similar motivation, regularizing by a contrastive loss to measure the distance between representations of the local model and the global model. Both methods add one more term to the loss function and require extra computations than FedAvg. SCAFFOLD \cite{karimireddy2019scaffold} adjusts the local gradient by keeping a correction term for each client, therefore its communication cost doubles. \citet{wang2021addressing} proposes to monitor the class imbalance of each client based on uploaded gradient together with a small public dataset. Then they mitigate the imbalance by their Ratio Loss. FedRS \cite{li2021fedrs} proposes to restrict the updates of missing classes by down-scaling their logits, however it only deals with missing classes. To further deal with minority classes, FedLC \cite{zhang2022federated} proposes to calibrate logits based on the label statistics of local training data. FedAlign \cite{mendieta2022local} proposes to add regularization terms during local training to learn well-generalized representations. FedOV \cite{diao2023towards} introduces the ``unknown'' class and trains open-set classifiers in local training for a better ensemble.  
%In some real-world applications such as mobile keyboard prediction, we may only need good personalized local models for the clients (e.g., mobile keyboard prediction). Personalized FL \cite{tan2022towards,Ghosh2020AnEF,fallah2020personalized,hanzely2020lower} has been a promising solution in this direction. 
More FL works and clustering techniques are discussed in Appendix A.1 and A.2. 

% \rev{More related works in FL are discussed in Appendix.}



% \YQ{We summarize these works in Table \ref{tbl:work}. These perspectives are all based on the averaging framework, which still suffers from label skews. Based on the averaging framework, it is difficult to locate the global optima for label skews. An opportunity is to deviate from averaging framework. Instead of approaching global optima, we attempt to utilize local optima of each client to construct a better global model.}

\iffalse
\begin{table*}[]
\centering
\caption{Comparison among improvements of some existing FL algorithms based on FedAvg \cite{mcmahan2016communication}.}
\label{tbl:work}
% \resizebox{0.8\columnwidth}{!}{
\begin{tabular}{|c|c|}
\hline
Pespective & Algorithms \\ \hline
\multirow{2}{*}{Improve local training} & FedProx \cite{lifedprox}, MOON \cite{li2021model}, \\
 & FedRobust \cite{reisizadeh2020robust}, SCAFFOLD \cite{karimireddy2019scaffold} \\ \hline
Revise server aggregation & FedNova \cite{wang2020tackling} \\ \hline
Client selection & Active FL \cite{Goetz2019ActiveFL} \\ \hline
% Personalized & IFCA \cite{Ghosh2020AnEF}, FeSEM \cite{Xie2020MultiCenterFL}, FL+HC \cite{Briggs2020FederatedLW}, FLT \cite{Rad2021FederatedLW} \\ \hline
\end{tabular}
% }
% \vspace{-20pt}
\end{table*}
\fi




% For more works on FL, one can refer to some surveys \cite{li2019flsurvey,litian2019survey,yang2019federated}. 

% \subsection{Personalized FL}
% In terms of clustering strategy, many works are from the perspective of personalized federated learning, where the aim is to train a good model for each client's data distribution, instead of only one global model for all clients. Although the goal of this work is to train a single joint model, their clustering methods can be integrated to our algorithm. For example, \cite{Ghosh2020AnEF} proposes to adaptively choose cluster membership for each client, by selecting the lowest loss model. Their IFCA framework sends multiply models in each round, and let each client to select its own membership. They have proved that selecting the model with lowest local loss can ensure effective convergence. \cite{Xie2020MultiCenterFL} adapts EM algorithm to FL setting and iteratively updates cluster center (i.e., cluster's global model) and membership in each communication round. Both works adapt cluster membership in each round, so they need considerable extra computation load. 

% There are also works only requiring one-time clustering. For example, \cite{Briggs2020FederatedLW} proposes to use hierarchical clustering based on each client's local update. It first performs FL among all clients for several rounds to get a decent global model, then uses local updates of the last round to perform clustering, and finally performs FL among each cluster to get a better model for specific cluster. \cite{Rad2021FederatedLW} utilizes a public pre-trained encoder to extract features of local data, then performs clustering in local features and submits cluster centers as signature of such client. The server evaluates the task relatedness of each pair of clients, based on their signature distance. Finally the task relatedness matrix is used to perform clustering, or to adjust weight of each client's update to other client. 

% \YQ{ Those personalized FL algorithms have a different goal from our paper. We aim to train a better global model, while they aim to train better models fit for different clients. Therefore, we need a new method to properly utilize the strength of each client's data. }




==> del/method.tex <==
\section{Our Method: FedConcat}

\subsection{Problem Statement}
Federated learning aims to train a global model on multiple clients without exposing their raw data. Denote $D^i$ the local dataset of client $i$. Suppose there are $K$ clients, and the local loss function for each client is $\mathcal{L}(\cdot,\cdot)$. Formally, our goal is to train a global model $f$ that minimizes the following objective.


\begin{equation}
    L = \frac{\sum_{i=1}^{K} |D^i|\cdot \mathbb{E}_{(X^i,Y^i)\sim D^i}[\mathcal{L}(f(X^i),Y^i)]}{\sum_{i=1}^{K} |D^i|}
    \label{eq:goal}
\end{equation}

\change{Like existing studies \citep{mcmahan2016communication, lifedprox, li2021model, karimireddy2019scaffold, wang2021addressing, li2021fedrs, zhang2022federated}, in this study, we assume that transmitting only models achieves a basic level of privacy protection in FL, compared with transferring the raw data. One can consider more advanced protection such as differential privacy (DP) to avoid inference attacks against the client models. Our method can be easily integrated with those privacy protection, which is not the focus of this paper and will be interesting future work. }

\subsection{Motivation}
\paragraph{Pitfalls of existing methods in label skews}
% While label skews are diverse in reality, it is challenging to directly take the degree of label skews into consideration when designing the FL approaches. Existing approaches~\cite{lifedprox,li2021model} usually introduce additional hyper-parameters to control the weight of the regularization term in local training to be adapted to different non-IID data settings. However, such hyper-parameters cannot directly quantify the influence of label skews on FL.
% Existing methods based on the averaging framework resort to alter the local training to avoid overfitting towards global optima under non-IID data distribution. However, it is hard to quantify the degree of heterogeneity to determine how much alteration to implement. We show the label distribution of real-world Criteo bidding dataset \cite{DiemertMeynet2017} in Figure \ref{fig:criteo}, which collects the bidding behavior of different clients. The label is whether the client bids or not for a product. As we can see, the label distribution varies among the clients. Some clients have almost all positive samples, while others have almost all negative samples. From the perspective of a client, it hardly knows how its label distribution differs from other clients. Even it knows, its local model can hardly be adapted to the global distribution based on its private data, especially when local label distribution is much different with global label distribution. 

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/criteo.pdf}
%     \caption{Label skews in the real-world Criteo dataset. }
%     \label{fig:criteo}
% \end{figure}

Under label skews, the local models can be much different as they are trained on different classes. Therefore it hardly makes sense to average each parameter of these models with quite different tasks. As an example, we train FedAvg on two clients of CIFAR-10 under label skews. The first client only has samples of class 0 and 2, while the second client only has samples of class 1 and 9. For both clients, we train 10 local epochs per round. We show the accuracy of local models and averaged global model of two rounds in Figure \ref{fig:track}. As we can see, the accuracy of local classes increases during local training, while the averaging operation leads to significant accuracy degradation. This example illustrates the problem of averaging local models under extreme label skews. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{figures/acc-track.pdf}
    \caption{Accuracy of local models and averaged model on two clients under label skews. }
    \label{fig:track}
\end{figure}

\paragraph{An alternative view of label skews}
Let us view the neural network as a feature extractor (all the layers in the network except the last layer
) and a classifier (the last layer). Since each client's model is well-fitted in its own dataset, we already have quite a few locally well-trained feature extractors. \YQ{Intuitively, concatenating the features from different local extractors can provide a better feature representation for label skews.} Thus we propose the idea of concatenating feature extractors and training a global classifier. 

%Training a global classifier for all features also needs FL algorithms like FedAvg \cite{mcmahan2016communication} to average those parameters. However, according to experimental results in \cite{li2021federated}, the label skew in MNIST dataset does not degrade the performance too much. This can be explained by the simplicity of MNIST dataset. If we directly perform FedAvg \cite{mcmahan2016communication} on the original dataset, we may need a complicated, non-linear global model to fit the dataset well, which is difficult to converge and can take many communication rounds. Now that we have extracted key features, a simple, linear global classifier may be enough to fit these key features well. We expect the global classifier is easy to converge. 

If we concatenate the models of all clients, our final model size can grow much large if there are many clients, and the overhead of training the global classifier is much more expensive. \rev{In practice, although label skews are prevalent, some parties may have similar label distributions. For example, hospitals in the same region may encounter similar types of diseases. } Therefore, we adopt the clustering method before training. By clustering all clients into a few groups via their label distributions, we can control the size of global model. Inside each group, since grouped clients have similar label distributions, the trained model can capture this kind of data well.

In brief, we tackle the label skew problem by generating solutions for each group individually. Next, we combine those solutions together to get a better global model with smaller communication cost. 

% \begin{figure*}[t]
%     \centering
%     \subfloat[Clustering stage: clients are clustered based on label distribution.]{\includegraphics[width=0.17\textwidth]{figures/1-new.png}}
%     \ \ \ \ 
%     \subfloat[Averaging stage: each cluster trains a model using FedAvg.]{\includegraphics[width=0.33\textwidth]{figures/2-new.png}}
%     \ \ \ \ 
%     \subfloat[Post-training stage: all well-trained feature extractors (E1, E2) are concatenated. All clients train a global classifier (C) collectively with feature extractors fixed.]{\includegraphics[width=0.44\textwidth]{figures/3-new.png}}
%     \caption{The workflow of FedConcat. For FedConcat-ID, label distributions are inferred in the clustering stage. }
%     \label{fig:alg}
% \end{figure*}

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\columnwidth]{figures/all-in.png}
    \caption{The workflow of FedConcat. (1) Clustering stage: clients are clustered based on label distributions; (2) Averaging stage: each cluster trains a model using FedAvg; (3) Post-training stage: all well-trained feature extractors (E1, E2) are concatenated. All clients train a global classifier (C) collectively with feature extractors fixed. For FedConcat-ID, label distributions are inferred in the clustering stage.}
    \label{fig:alg}
    % \vspace{-10pt}
\end{figure}

\subsection{Proposed Algorithm}
% Suppose there are $N$ clients and we divide them into $K$ clusters. Denote the encoder of cluster $i$ as $E_i$ and its classifier as $C_i$. Suppose each raw data has $d_i$ dimensions, the embedding space has $d_e$ dimensions and there are $d_o$ classes in total. Thus, each $E_i$ maps $\mathbb{R}^{d_i}$ into $\mathbb{R}^{d_e}$ and each $C_i$ maps $\mathbb{R}^{d_e}$ into $\mathbb{R}^{d_o}$. 

% After performing some FL algorithm among each cluster, we concatenate $\{E_1,E_2,...,E_{K}\}$ as a global encoder $E: \mathbb{R}^{d_i} \rightarrow \mathbb{R}^{Kd_e}$ and fix its parameters. Then we train a global classifier $C: \mathbb{R}^{Kd_e} \rightarrow \mathbb{R}^{d_o}$ collaboratively among all clients. 

Our framework is illustrated in Figure \ref{fig:alg}. It has three stages: clustering, averaging and post-training. First, clients with similar label distributions are grouped into same cluster. Then, each cluster performs FL to train a model that fits well inside the cluster. Finally, the server collects feature extractors of all clusters with their parameters fixed, and train a global classifier among all clients. The overall algorithm is shown in Algorithm \ref{alg:new}. In the following, we elaborate those stages in detail. 

\paragraph{Stage 1-A: Clustering with label distributions}
In order to alleviate the label imbalance problem, we perform clustering based on label distributions, so that each cluster hosts clients with similar label distributions. Formally, for client $i$, suppose there are $N_{i,j}$ samples of class $j$, and there are a total of $N_i = \sum_j N_{i,j}$ samples. Its label distribution is defined as vector
\begin{equation}
    P_i(y)=(\frac{N_{i,1}}{N_i},\frac{N_{i,2}}{N_i},...,\frac{N_{i,m}}{N_i} ) ,
    \label{eq:lb}
\end{equation}
where there are $m$ classes globally. In this paper, we use K-means algorithm \cite{Lloyd1982LeastSQ} to perform clustering for its popularity and simplicity. For the hyper-parameter $K$, one can utilize elbow method to select the best value. For simplicity, we use K-means for clustering as it is popular and sufficiently good for our study. We have also tried other clustering methods, which are presented in Section \ref{sec:main_cfl}. \rev{With clustering, we can control the number of different models generated by the clients, which helps to reduce the model size in our later concatenation.}

\paragraph{Stage 1-B: Clustering without label distributions}
If clients are unable to upload label distributions due to privacy concerns, we propose to utilize the uploaded local models of the first round to infer the approximate label distribution of each client. \rev{In this way, we only upload trained models like FedAvg, which does not cause any extra privacy leakage.}

\rev{During local training, if a class appears more frequently, the model is prone to output a higher probability for that class. Many works \cite{johnson2019survey, bahng2020learning} have observed that predictions of deep learning model are biased towards the majority classes of the training set.} Intuitively, if we put a large batch of random inputs into the client model, the average prediction can indicate the label distribution of training data. Thus, we generate random data (i.e., images that each pixel is randomly generated from range zero to one) and
% Another problem is to estimate a reasonable range for random inputs. A solution is to first normalize each feature, and then generate random inputs by normal distribution. To calculate the mean and variance of each feature, one can utilize existing multi-party computation methods \cite{cramer2001multiparty,cramer2003efficient} to protect privacy. 
% Now that the random inputs are in the similar range of features, 
input these random data into each client model. Then, we calculate the average prediction probability for each class as the inferred label distribution of each client. Formally, denote the model of client $i$ as $f_i$. We randomly generate $r$ inputs $X_1,...,X_r$, the inferred distribution of client $i$
\begin{equation}
P_{i}^{ID}(y)=\frac{1}{r} \sum_{j=1}^r \sigma(f_i(X_j)),
    \label{eq:id}
\end{equation}
where $\sigma$ is the softmax function.

\change{We refer to this variant as FedConcat with Inferred Distribution (FedConcat-ID). A neural network classifier can be viewed as a function $p(Y|X)$ learned on its training data. In an ideal scenario, if the inputs $X$ are independent of $Y$, the equation $p(Y)=p(Y|X)$ holds true. The underlying intuition of Eq. \ref{eq:id} is to employ uninformative inputs to approximate $p(Y)$. }

% \change{During implementation, we can aggregate the uploaded models among each cluster as the first round (Line 7 in Algorithm \ref{alg:new}).}

% \change{We refer to this variant as FedConcat with Inferred Distribution (FedConcat-ID). To demonstrate the effectiveness of our inference, we compare our label inference results with ground truth and other methods, as detailed in Appendix \ref{sec:more_exp_concat_id}. }

% \change{FedConcat-ID only transfers models, which achieves the same privacy guarantee as FedAvg. While inferring label distribution can be viewed as inference attack, our approach only estimates the approximate label distributions instead of raw data in typical inference attack studies \cite{zhu2019deep, wang2019beyond}. More discussions of privacy are in Appendix \ref{sec:privacy_analysis}. }
% Besides FedConcat-ID, applying differential privacy \cite{dwork2011differential,dwork2014algorithmic} is another solution to protect the label distributions, as shown in Appendix \ref{sec:dp}.
%For implementation, since we experiment on image datasets and all pixels are pre-processed in the range of $[0,1]$, we generate 10,000 random images with each pixel uniformly randomly chosen in $[0,1]$. Then we input these random images into each client model, and calculate the average prediction probability for each class as inferred label distribution of such client. 

\paragraph{Stage 2: Averaging}
Within each cluster, we use FedAvg \cite{mcmahan2016communication} to train a model that fits well for such cluster. \YQ{Inside a cluster, since the label distributions of the clients are similar, we expect the global model to have a good performance on the dominant classes of the cluster.} 
% One can also consider other FL algorithms for averaging like FedProx \cite{lifedprox} or MOON \cite{li2021model}. 

\paragraph{Stage 3: Post-training}
Now that we have $K$ models, we stack their encoders (all layers but the last layer) as the global feature extractor. Then we broadcast the global feature extractor to all clients for one time, and ask clients to jointly train a classifier using FedAvg, with the global feature extractor fixed. Since the encoder training is stopped, we can calculate the features of raw data in a forward pass for only one time. For other training rounds, we can directly feed features into the linear classifier to train it. Therefore in this stage, our major computation and communication happens only for the linear classifier. 

% Compared with training on all parameters, fixing the parameters of encoders achieve comparable accuracy with much smaller communication cost, as shown in Section \ref{sec:large-model}. Moreover, under label skews, FedConcat has much more stable training curves than baselines on large model. 

% Fixing the parameters of encoders can be viewed as a trade-off between accuracy and communication cost. We show such trade-off by experiments in Section \ref{sec:large-model}. Directly training on all parameters can obviously have better representation than fixing them. However, our method can achieve comparable accuracy with much smaller communication cost. Moreover, under label skew cases, FedAvg on large model has unstable training curve, while FedConcat is much more stable.
% where we use FedAvg \cite{mcmahan2016communication} to train models of each cluster and the final global classifier.



\begin{algorithm}[ht]
\SetNoFillComment
\LinesNumbered
\SetArgSty{textnormal}
\KwIn{number of clients $N$, number of clusters $K$, number of training rounds of the encoder $T_e$, number of training rounds of the classifier $T_c$}
\KwOut{the final model $w$}
%\BlankLine
%\tb{Server executes}:
% \If {FedConcat}{
% Ask for the label distribution of each client (Equation \ref{eq:lb}) and perform K-means algorithm to divide $N$ clients into $K$ clusters

% Initialize encoder $E_i$ and classifier $C_i$ of cluster $i$ for $i=1,2,...,K$
% }
% \If {FedConcat-ID}{
% Initialize one encoder and one classifier and send the models to clients for local training

% Infer client label distribution based on received local models (Equation \ref{eq:id}), and perform K-means to divide $N$ clients into $K$ clusters

% The client models are then averaged to get $E_i$ and $C_i$ of the first round for each cluster $i$
% }

% % FedConcat: ask for the label distribution of each client (Equation \ref{eq:lb}), and perform K-means algorithm to divide $N$ clients into $K$ clusters. Initialize encoder $E_i$ and classifier $C_i$ of cluster $i$ for $i=1,2,...,K$. 

% % FedConcat-ID: initialize one encoder and one classifier for all clients. Send the models to clients for local training. After receiving local models, infer the client distribution (Equation \ref{eq:id}), and perform K-means algorithm to divide $N$ clients into $K$ clusters. The client models are then averaged to get $E_i$ and $C_i$ of the first round for each cluster $i$.

% \For {$t=1,2,..., T_e$}{
%     \For {$i=1,2,...,K$}{
%     Run FedAvg on clients of cluster $i$ to train $E_i$ and $C_i$ (FedConcat-ID: start with $t=2$ as the first round is already done)
% }
% }

% Initialize global encoder $E=\{E_1,E_2,...,E_{K}\}$ and global classifier $C$
 
% \For {$t=1,2, ..., T_c$}{
%     Fix $E$ and run FedAvg on all clients to train $C$
% }

% \Return final model $w=\{E, C\}$

\If {FedConcat}{
% Get the label distribution of each client and perform K-means clustering
$S_1, S_2, ..., S_K \leftarrow Kmeans({P_i(y)}_{i=1}^N)$ {// Perform K-means based on label distributions}
}
\If {FedConcat-ID}{
Initialize global model $f_g$

\For {$i=1,2,...,N$ in parallel} {
$f_i \leftarrow TrainLocal(f_{g})$ // Send model to each client for local training}

% Infer client label distribution based on local models and perform K-means clustering
$S_1, S_2, ..., S_K \leftarrow Kmeans({P_{i}^{ID}(y)}_{i=1}^N)$ {// Infer label distributions (Eq. \ref{eq:id}) and perform K-means}

}

Initialize encoder $E_i$ and classifier $C_i$ for each cluster

\For {$t=1,2,..., T_e$}{
\For {$i=1,2,...,K$}{
$E_i, C_i \leftarrow FedAvg(\{E_i, C_i\}, S_i)$ // {Run FedAvg to train encoder and classifier for each cluster}
}
}

$E=\{E_1,E_2,...,E_{K}\}$ 

Initialize global classifier $C$

\For {$t=1,2, ..., T_c$}{
$C \leftarrow FedAvg(C, \bigcup_{i=1}^{K}S_i)$ // {Fix $E$ and run FedAvg on all clients to train $C$}
}

\Return final model $w=\{E, C\}$

\caption{FedConcat and FedConcat-ID}
\label{alg:new}
\end{algorithm}

% \begin{algorithm}[ht]
% \SetNoFillComment
% \LinesNumbered
% \SetArgSty{textnormal}
% \KwIn{number of clients $N$, number of clusters $K$, number of training rounds of the encoder $T_e$, number of training rounds of the classifier $T_c$}
% \KwOut{final model $w$}

% \If {FedConcat}{
% % Get the label distribution of each client and perform K-means clustering
% $S_1, S_2, ..., S_K \leftarrow Kmeans({P_i(y)}_{i=1}^N)$\tcp*{Perform K-means based on label distributions}

% Initialize encoders and classifiers $\forall i: 1\leq i \leq K: E_i, C_i \leftarrow Init()$\tcp*{Initialize encoder and classifier for each cluster}
% }
% \If {FedConcat-ID}{
% Initialize global models $E_{global}, C_{global} \leftarrow Init()$\tcp*{Initialize one encoder and classifier}

% Send models to clients for local training: $\forall n: 1\leq n \leq N: E_n, C_n \leftarrow TrainLocal(E_{global}, C_{global})$\tcp*{Send models for local training}

% % Infer client label distribution based on local models and perform K-means clustering
% $S_1, S_2, ..., S_K \leftarrow Kmeans({P_{id_n}(y)}_{n=1}^N)$\tcp*{Infer label distributions and perform K-means}

% $\forall i: 1\leq i \leq K: E_i, C_i \leftarrow \frac{1}{|S_i|}\sum_{n \in S_i}E_n, C_n$\tcp*{Average local models per cluster}
% }

% \For {$t=1,2,..., T_e$}{
% \For {$i=1,2,...,K$}{
% $E_i, C_i \leftarrow FedAvg(E_i, C_i, S_i)$\tcp*{Run FedAvg to train encoder and classifier for each cluster}
% }
% }

% Initialize global encoder and classifier: $E={E_1,E_2,...,E_{K}}, C \leftarrow Init()$

% \For {$t=1,2, ..., T_c$}{
% Fix $E$ and $C \leftarrow FedAvg(C, E, \bigcup_{i=1}^{K}S_i)$\tcp*{Fix $E$ and run FedAvg on all clients to train $C$}
% }

% \Return final model $w={E, C}$

% \caption{FedConcat and FedConcat-ID}
% \label{alg:new}
% \end{algorithm}

% Both FedConcat and FedConcat-ID can reduce the communication cost by limiting the encoder training rounds $T_e$. For classifier training, clients only need to update and communicate the last layer. 


\section{Theoretical Analysis and Discussion}

\subsection{Analyzing FedConcat by Information Bottleneck}
To answer the question why concatenating encoders works for extreme label skews, we refer to the information bottleneck theory \cite{shwartz2017opening}. Suppose a deep neural network $f$ is trained on dataset $D$. Denote a random train sample $(X,Y) \sim D$ where $X$ are input variables and $Y$ are desired outputs. Suppose the extracted features (representation before the last fully-connected layer) is $Z$, the neural network learns an encoder which minimizes 
\begin{equation}
   \mathbf{E}_{(X,Y)\sim D} [I(X;Z)-\beta I(Z;Y)],
\end{equation}
where $I(\cdot;\cdot)$ denotes the mutual information between two variables and $\beta$ is a positive trade-off parameter related to the task. 

In brief, the encoder of deep neural network aims to remember the features related to the target outputs (maximizing $I(Z;Y)$), while forgetting the information of inputs unrelated to the target outputs (minimizing $I(X;Z)$). 

Consider the label skews in federated learning. Suppose there are two clients with local datasets $D^1$ and $D^2$ respectively. Their locally trained encoders are $f_{e1}$ and $f_{e2}$. Denote the FedConcat encoder as $f_e(\cdot)=\{f_{e1}(\cdot), f_{e2}(\cdot)\}$ and the FedAvg encoder as $f_{avg}$. We have the following theorem.

\begin{theorem}
    $I(f_{avg}(X);Y) < I(f_{e}(X);Y)$, $\forall (X,Y)\sim D^1 \cup D^2$.
\end{theorem}

\begin{proof}
According to the information bottleneck theory, the local model of the first client minimizes
\begin{equation}
   \mathbf{E}_{(X^1,Y^1)\sim D^1} [I(X^1;f_{e1}(X^1))-\beta_1 I(f_{e1}(X^1);Y^1)].
\end{equation}

Similarly, the second client's local model minimizes
\begin{equation}
   \mathbf{E}_{(X^2,Y^2)\sim D^2} [I(X^2;f_{e2}(X^2))-\beta_2 I(f_{e2}(X^2);Y^2)].
\end{equation}

For a good global encoder $f_e$, it should minimize
\begin{equation}
   \mathbf{E}_{(X,Y)\sim D^1 \cup D^2} [I(X;f_{e}(X))-\beta I(f_{e}(X);Y)].
\end{equation}

For the mutual information between representation and target, no matter whether $(X,Y) \sim D^1$ or $(X,Y) \sim D^2$, we have 
\begin{equation}
    I(f_{e}(X);Y) \geq \max\{I(f_{e1}(X);Y), I(f_{e2}(X);Y)\},
\end{equation}
which means the representation of concatenated encoders are more related to the global targets than single locally optimized encoder. 

For the part of forgetting task-unrelated information, we have
\begin{equation}
    I(f_{e}(X);X) \geq \max\{I(f_{e1}(X);X), I(f_{e2}(X);X)\},
\end{equation}
which is a disadvantage according to information bottleneck theory. However, under extreme label skews, the encoder of a client can extract little information related to data of another client. According to experimental results in \citet{shwartz2017opening}, when deep neural network reaches convergence, the mutual information between last layer representation and raw input (i.e. $I(f_e(X);X)$) becomes very small, as compared to $I(f_e(X);Y)$. Therefore, we regard $I(f_e(X);Y)$ as the main part. We also justify such hypothesis by experiments, which are included in Appendix C.

For the averaging solution, under label skews, the averaged global model becomes very different from local optima. Thus, for $(X,Y) \sim D^1$, we have %however, we cannot explain the operation of averaging model parameters from the perspective of information theory. When label skews are significant and local optima of different clients are far away, %one has to set smaller local step, which leads to slower convergence. 
\begin{equation}
    I(f_{avg}(X);Y) < I(f_{e1}(X);Y) \leq I(f_{e}(X);Y).
    \label{eq:10}
\end{equation}

Similarly, for $(X,Y) \sim D^2$, we have
\begin{equation}
    I(f_{avg}(X);Y) < I(f_{e2}(X);Y) \leq I(f_{e}(X);Y).
    \label{eq:11}
\end{equation}

Combining Eq. \ref{eq:10} and \ref{eq:11}, for $(X,Y)\sim D^1 \cup D^2$, we have 
$I(f_{avg}(X);Y) < I(f_{e}(X);Y)$.

\end{proof}

\paragraph{Implication} Under label skews, the averaged encoder contains less mutual information about the labels compared with the concatenation of well-trained local encoders. This explains why the averaged model suffers from accuracy decay compared with local models, as shown in Figure \ref{fig:track}.

\subsection{Privacy}
\change{FedConcat needs client label distribution information, therefore it is applicable when local label distribution is not sensitive. For scenarios that also consider label distribution privacy, users can adopt FedConcat-ID, which only transfers the models and provides the same privacy level as FedAvg. The inference attack towards client model is a complex topic and defense mechanisms against them fall outside this paper's scope. It is an interesting topic to explore more robust measures to prevent such breaches in future works.}

% \change{Contrasting our methods with FedAvg, two salient privacy-related aspects need clarification. Firstly, FedConcat and FedConcat-ID broadcast cluster encoders not only to the server but also to all clients. This raises concerns about an enhanced risk of privacy leakage due to the increased number of recipients. Secondly, FedConcat-ID infers label distributions from the model, which could be interpreted as an inference attack, introducing potential vulnerabilities concerning the leakage of local label distributions.}

% \change{For the first issue, we recognize the inherent risk in broadcasting the global feature extractor to all clients. While our system predicates on the assumption that all involved parties are honest but curious, meaning they do not maliciously misuse the data but may be curious about its content, we admit this broadcasting could be a potential source of vulnerability. Prior works addressing non-IID problems \citep{mcmahan2016communication, lifedprox, li2021model, karimireddy2019scaffold, wang2021addressing, li2021fedrs, zhang2022federated} also involve model uploads and do not directly tackle the model inference attack problem. This is a significant area for future research and investigation. The potential risk is mainly associated with the nature of client-uploaded information, not just the number of recipients. Still, it is important to ensure a robust system where feature broadcasting minimally affects privacy.}

% \change{Regarding the second point, FedConcat-ID maintains privacy similar to FedAvg by only uploading models. Though the global model is accessible to all, actual local label distributions are not. Most existing inference attack studies, such as \cite{zhu2019deep, wang2019beyond}, aim to derive raw data, not label distributions. We agree that the potential for inference attacks is a complex topic and defense mechanisms against them fall outside this paper's scope. It is an interesting topic to explore more robust measures to prevent such breaches in future works.}
% \change{Compared with FedAvg, there are two points to clarify privacy of FedConcat and FedConcat-ID. First, FedConcat and FedConcat-ID broadcast cluster encoders to not only the server but also all clients. Some readers may have concern that the extra recipients lead to more privacy leakage. Second, FedConcat-ID infers label distributions from the model. Some readers may regard it as inference attack and concern the leakage of local label distributions. }

% \change{For the first question, we do not agree that the privacy leakage risk increases with more recipients, because the server cannot be trusted to keep the uploaded information. We assume that the server and clients are honest but curious like in \cite{fang2020highly, bonawitz2016practical, hu2021source}. Since the server can leak the uploaded information to others, the information leakage depends on the uploaded information from clients, while not quite related to whether other parties receive the information. For example, to prevent insider trading, no sensitive information is allowed to share to any outside person. Regulations focus the disclosed information itself, rather than how many parties receive it.}

% \change{For the second question, FedConcat-ID achieves the same privacy guarantee as FedAvg, where all clients and the server have access to the global model and no access to true local label distributions. Inference attacks and defenses on the models are out of scope of the paper. Besides, typical inference attack studies \cite{zhu2019deep, wang2019beyond} aim to infer raw data instead of label distributions. }


\subsection{Communication}

Suppose the model size is $w$, and its last classifier layer size is $cw$ ($c<1$). For $T_e$ encoder rounds, each client's communication cost is $2T_ew$. Downloading the concatenated model costs $Kw$. Next, for classifier rounds each client costs $2T_cKcw$. The total cost of FedConcat is $2wN(T_e+K/2+cKT_c)$. For FedAvg with $T$ rounds, the cost is $2wNT$. Suppose $T=T_e+T_c$ (i.e., we train the same communication rounds for FedAvg and FedConcat). Given the same model size $w$ and the number of clients $N$, communication overhead can be saved by choosing small $c,K$, i.e. limiting the classifier size and number of cluster. Experimental results of accuracy with respect to communication cost are shown in Appendix D.2. \change{Our approach achieves higher accuracy and more stable convergence given the same communication cost with FedAvg and other baselines.}
